Performance-Driven Optimization of Parallel Breadth-First Search

Breadth-first search (BFS) is a fundamental graph algorithm that presents significant challenges for parallel implementation due to irregular memory access patterns, load imbalance and synchronization overhead. In this paper, we introduce a set of optimization strategies for parallel BFS on multicore systems, including hybrid traversal, bitmap-based visited set, and a novel non-atomic distance update mechanism. We evaluate these optimizations across two different architectures - a 24-core Intel Xeon platform and a 128-core AMD EPYC system - using a diverse set of synthetic and real-world graphs. Our results demonstrate that the effectiveness of optimizations varies significantly based on graph characteristics and hardware architecture. For small-diameter graphs, our hybrid BFS implementation achieves speedups of 3-8x on the Intel platform and $3-10\times$ on the AMD system compared to a conventional parallel BFS implementation. However, the performance of large-diameter graphs is more nuanced, with some of the optimizations showing varied performance across platforms including performance degradation in some cases.

==> codes_golden.tex <==



\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_naive,caption=BFS(sir code)]
  |\vspace{0.65em}\tikzmarkin[set fill color=grayblack, set border color=white, above offset=0.25, below offset=-0.1]{bl1} \textcolor{white}{/*\quad\quad\quad\quad\quad\quad  Threads spawned every iteration */ \quad\quad\quad\quad\quad\quad} \tikzmarkend{bl1}|
  // fsz: frontier size, lfsz: local frontier size
  while (fsz != 0) {
    #pragma omp parallel for schedule(runtime) nowait
    for (uint32_t i = 0; i < fsz; ++i) {
      vidType src = frontier[cur][i];
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) 
      {
        vidType dst = col[j];
        if (dist[src] + 1 < dist[dst]) {
          dist[dst] = dist[src] + 1;
          // Add to local frontier
          lf[lfsz++] = dst;
        }
      }
    }
    if (lfsz != 0) {
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        frontier[1-cur][fstart+i] = lf[i];
    }
    #pragma omp barrier
    cur = 1 - cur;
    #pragma omp single {
      cfsz = nxt_fsz;
      nxt_fsz = 0;
    }
    lfsz = 0;
  }
  \end{lstlisting}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 0 // //Pure Top-Down with Locks, thread launched every iteration
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if 0
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v0,caption=BFS(Threads Launched every iteration)]
|\vspace{0.65em}
% \tikzmarkin[set fill color=grayblack, set border color=white, above offset=0.25, below offset=-0.1]{bl1} \textcolor{white}{/*\quad\quad\quad\quad\quad\quad  Threads spawned every iteration */ \quad\quad\quad\quad\quad\quad} \tikzmarkend{bl1}
|
// cfsz: frontier size, lfsz: local frontier size
while (cfsz != 0) {
  #pragma omp parallel
  {  //conventional Top-down step
    //Traverse all vertices in current frontier
    #pragma omp for nowait
    for (uint32_t i = 0; i < cfsz; ++i) {
      vidType src = curr_frontier[i];
      //Traverse all neighbors of frontier vertex
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
        vidType dst = col[j];
        //if neighbor is not visited
        if (dist[src] + 1 < dist[dst]) {
          //atomically update the neighbor's distance
          weight_type max_dist = std::numeric_limits<weight_type>::max()
          if (__sync_bool_compare_and_swap(&dist[dst], max_dist, dist[src] + 1)) {
            // Add to local frontier
            lf[lfsz++] = dst;
          }
        }
      }
    }
    if (lfsz != 0) {
      // nxt_fsz: next frontier size
      // collect local frontiers into next frontier
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        next_frontier[fstart+i] = lf[i];
    }  
  }
  swap(curr_frontier, next_frontier);
  fsz = nxt_fsz;
  nxt_fsz = 0;
}
\end{lstlisting}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 1 //Pure Top-Down with Locks, thread launched only once
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v1,caption=BFS(Threads launched only once)]
#pragma omp parallel
{
  w_type max_dist = numeric_limits<w_type>::max();
  while (cfsz != 0) {
    // Traverse all vertices in current frontier
    #pragma omp for nowait
    for (uint32_t i = 0; i < cfsz; ++i) {
      vidType src = curr_frontier[i];
      // Traverse all neighbors of frontier vertex
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
        vidType dst = col[j];
        // if neighbor is not visited
        if (dist[src] + 1 < dist[dst]) {
          // |\color{darkred}{BFS-Traditional: atomically update the neighbor's distance}|
          |\vspace{-0.8em}|
          |\vspace{0.8em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=4.1]{codebox}
          if (\_\_sync\_bool\_compare\_and\_swap(\&dist[dst], max\_dist, dist[src] + 1)) \{
          \tikzmarkend{codebox} |

          // |\color{darkred}{BFS-NonAtomic: Update the distance directly}|
          |\vspace{0.4em} \tikzmarkin[set fill color=lightblue, set border color=white, above offset=0.22, below offset=-0.1, right offset=3.62]{codebox3}
          dist[dst] = dist[src] + 1;
          \tikzmarkend{codebox3} |

            // Add to local frontier
            lf[lfsz++] = dst;
          |\vspace{0.6em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=6.6]{codebox2}
          \}
          \tikzmarkend{codebox2} |
        }
      }
    }
    if (lfsz != 0) {
      // collect local frontiers
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        next_frontier[fstart+i] = lf[i];
    }
    #pragma omp barrier
    
    #pragma omp single
    {
      swap(curr_frontier, next_frontier);
      fsz = nxt_fsz; nxt_fsz = 0;
    }
    lfsz = 0;
  }
}
\end{lstlisting}

\if 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 2 //Pure Top-Down without Locks, thread launched only once
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v2,caption=BFS(Removed locks allowing Duplicates)]
//only change is-  if condition at line 15 of previous version is removed
//removed locks at the cost of some redundant work
#pragma omp parallel
{
  while (cfsz != 0) {
    // Traverse all vertices in current frontier
    #pragma omp for nowait
    for (uint32_t i = 0; i < cfsz; ++i) {
      vidType src = curr_frontier[i];
      // Traverse all neighbors of frontier vertex
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
        vidType dst = col[j];
        // if neighbor is not visited
        if (dist[src] + 1 < dist[dst]) {
          //update the neighbor's distance
          dist[dst] = dist[src] + 1;
          // Add to local frontier
          lf[lfsz++] = dst;
        }
      }
    }
    if (lfsz != 0) {
      // collect local frontiers
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        next_frontier[fstart+i] = lf[i];
    }
    #pragma omp barrier
    
    #pragma omp single
    {
      swap(curr_frontier, next_frontier);
      fsz = nxt_fsz;
      nxt_fsz = 0;
    }
    lfsz = 0;
  }
}
    
\end{lstlisting}
\fi
% \FloatBarrier
% => As shown in Plot 4 on Notion, pure top-down without locks(version 2) is the best performing version for large diameter graphs 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Botttomup step algorithm from scot beamer 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em,
float=!h, label=lst:bfs_bottom_up, caption=Bottom-Up Step]
  //curr_front_bm: current frontier bitmap
  //nxt_front_bm: next frontier bitmap
  void BottomUpStep( curr_front_bm, nxt_front_bm, distances) {
    // Traverse all vertices
     #pragma omp for nowait reduction(+: nxt_fsz)
    for (vidType v = 0; v < N; v++) { 
      // If v is unvisited
      if (distances[v] == MAX_DISTANCE) { 
        //traverse all its neighbors
        for (uint32_t i = rptr[v]; i < rptr[v + 1]; ++i) {
          vidType neighbor = col[i];
          // Check if its neighbors are in current frontier
          if (curr_front_bm[neighbor]) {
            distances[v] = depth + 1;
            nxt_fsz++;
            nxt_front_bm[v] = true;
            break;
          }
        }
      }
    }
  }
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 3 //Hybrid(Top-Down + Bottom-Up)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v3,caption=BFS(Hybrid approach implemented by scott beamer)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      //Top-down step including counting next frontier edges
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz; ++i) {
        vidType src = curr_frontier[i];
        for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
          vidType dst = col[j];
          if (dist[src] + 1 < dist[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
            //lfe: local frontier edges
            lfe += rptr[dst + 1] - rptr[dst];
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
      #pragma omp single
      {   
        visited_edges += frontier_edges;
        frontier_edges = 0;
      }
      #pragma omp atomic
      frontier_edges += lfe;
    }
    else{
      // reset next frontier bitmap
      #pragma omp for
      for(uint32_t v = 0; v < N; v++)
        nxt_front_bm[v] = false;
      BottomUpStep( curr_front_bm, nxt_front_bm, distances)
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      unvisited_edges  =  M - visited_edges;
      is_top_down = scot_beamer_switching_criterion(visited_edges, unvisited_edges, frontier_edges, M);
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 4 // Hybrid modified switching criteria
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v4,caption=BFS(Modified switching criteria)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      //only Top-down step(no need of extra work)
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz; ++i) {
        vidType src = curr_frontier[i];
        for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
          vidType dst = col[j];
          if (dist[src] + 1 < dist[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
    }
    else{
      // reset next frontier bitmap
      #pragma omp for
      for(uint32_t v = 0; v < N; v++) 
        nxt_front_bm[v] = false;
      BottomUpStep( curr_front_bm, nxt_front_bm, distances)
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      //switch to BU if frontier size > 5% of #vertices
      is_top_down = (curr_frontier_size > 0.05 * N)? true : false ;
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v5,caption=BFS(using visited\_bitmap)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz; ++i) {
        vidType src = curr_frontier[i];
        for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
          vidType dst = col[j];
          //check if a neighbor is already visited using a bitmap
          if (!visited_bitmap[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
            visited_bitmap[dst] = true;
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
    }
    else{
      #pragma omp for nowait reduction(+: nxt_fsz)
        for (vidType v = 0; v < N; v++) { 
          //check if a vertex is unvisited using a bitmap
          if (!visited_bitmap[v]) { 
            for (uint32_t i = rptr[v]; i < rptr[v + 1]; ++i) {
              vidType neighbor = col[i];
              if (curr_front_bm[neighbor]) {
                distances[v] = depth + 1;
                nxt_fsz++;
                nxt_front_bm[v] = true;
                visited_bitmap[v] = true;
                break;
              }
            }
          }
        }
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      is_top_down = (curr_frontier_size > 0.05 * N)? true : false ;
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 6
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v6,caption=BFS(Loop Unrolling)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz / 4 * 4; i += 4) { 
        vidType src1 = curr_frontier[i];
        vidType src2 = curr_frontier[i + 1];
        vidType src3 = curr_frontier[i + 2];
        vidType src4 = curr_frontier[i + 3];

        for (uint32_t j = rptr[src1]; j < rptr[src1 + 1]; ++i) {
          vidType dst = col[j];
          if (dist[src1] + 1 < dist[dst]) {
            dist[dst] = dist[src1] + 1;
            lf[lfsz++] = dst;
          }
        }
        for (uint32_t j = rptr[src2]; j < rptr[src2 + 1]; ++i) {
          vidType dst = col[j];
          if (dist[src2] + 1 < dist[dst]) {
            dist[dst] = dist[src2] + 1;
            lf[lfsz++] = dst;
          }
        }
        for (uint32_t j = rptr[src3]; j < rptr[src3 + 1]; ++i) {
          vidType dst = col[j];
          if (dist[src3] + 1 < dist[dst]) {
            dist[dst] = dist[src3] + 1;
            lf[lfsz++] = dst;
          }
        }
        for (uint32_t j = rptr[src4]; j < rptr[src4 + 1]; ++i) {
          vidType dst = col[j];
          if (dist[src4] + 1 < dist[dst]) {
            dist[dst] = dist[src4] + 1;
            lf[lfsz++] = dst;
          }
        }
      }
      // Handle the remainder of the loop
      #pragma omp for schedule(static) nowait
      for (uint32_t idx = (cfsz / 4) * 4; idx < cfsz; ++idx) {
        vidType src = curr_frontier[idx];
        for (uint32_t i = rptr[src]; i < rptr[src + 1]; ++i) {
          vidType dst = col[i];
          if (dist[src] + 1 < dist[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
    }
    else{
      #pragma omp for nowait reduction(+: nxt_fsz)
        for (vidType v = 0; v < N; v++) { 
          //check if a vertex is unvisited using a bitmap
          if (dist[v] == MAX_DISTANCE) { 
            for (uint32_t i = rptr[v]; i < rptr[v + 1]; ++i) {
              vidType neighbor = col[i];
              if (curr_front_bm[neighbor]) {
                dist[v] = depth + 1;
                nxt_fsz++;
                nxt_front_bm[v] = true;
                visited_bitmap[v] = true;
                break;
              }
            }
          }
        }
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      is_top_down = (curr_frontier_size > 0.05 * N)? true : false ;
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 7
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v7,caption=BFS(simd)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz; ++i) {
        vidType src = curr_frontier[i];
        for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
          vidType dst = col[j];
          if (dist[src] + 1 < dist[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
    }
    else{
      #pragma omp for schedule(static) nowait reduction(+: nxt_fsz)
      for(uint32_t v = 0; v < N; v++){
        __m256i depth_vec = _mm256_set1_epi32(depth);
        if(distances[v] == MAX_DISTANCE) {
          bool is_parent = false;
          uint32_t i_end = rptr[v] + ((rptr[v + 1] - rptr[v]) / chunksize) * chunksize;
          for (uint32_t i = rptr[v]; i < i_end; i += chunksize) {
            _mm_prefetch((const char*)&col[i + chunksize], _MM_HINT_T0);
            _mm_prefetch((const char*)&curr_frontier_bm[col[i + chunksize]], _MM_HINT_T0);
            // __mmask16 mask = 0;
            for (uint32_t j = i; j < i + chunksize; j += 8) {
              // _mm_prefetch((const char*)&col[j + 16], _MM_HINT_T0);
              // __m512i indices = _mm512_loadu_si512((__m512i*)&col[j]);
              // _mm_prefetch((const char*)&curr_frontier_bm[col[j + 16]], _MM_HINT_T0);
              // __m512i curr_frontier_bm_values = _mm512_i32gather_epi32(indices, (const int*)curr_frontier_bm, 1);
              
              __m256i parent_vec = _mm256_loadu_si256((__m256i*)&col[j]);
              __m256i distances_vec = _mm256_i32gather_epi32((int const*)dist, parent_vec, 4);                          
              __m256i cmp_result = _mm256_cmpeq_epi32(distances_vec, depth_vec);
              if (_mm256_movemask_epi8(cmp_result)) {
                is_parent = true;
              }
            }
            if(is_parent) {
              distances[v] = depth + 1;
              nxt_fsz++;
              next_frontier_bm[v] = true;
              //is_parent = true;
              break;
            }
          }
          for (uint32_t i = i_end; i < rptr[v + 1]; i++) {
            vidType neighbor = col[i];
            if(curr_frontier_bm[neighbor]) {
              distances[v] = depth + 1;
              nxt_fsz++;
              next_frontier_bm[v] = true;
              break;
            }
          }
        }
      }
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      is_top_down = (curr_frontier_size > 0.05 * N)? true : false ;
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 8
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=1em, belowskip=-2.5em, float=!h,label=lst:bfs_v8,caption=BFS(Flushing)]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down){
      #pragma omp for nowait
      for (uint32_t i = 0; i < cfsz; ++i) {
        vidType src = curr_frontier[i];
        for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
          vidType dst = col[j];
          if (dist[src] + 1 < dist[dst]) {
            dist[dst] = dist[src] + 1;
            lf[lfsz++] = dst;
            //check if local frontier is full
            if(lfsz == max_lfsz){
              //flush to global frontier
              f_start = __atomic_fetch_add(&next_frontier_size, lfsz, __ATOMIC_SEQ_CST);
              for (uint32_t i = 0; i < lfsz; ++i) {
                next_frontier[f_start + i] = lf[i];
              }
              lfsz = 0;
            }
          }
        }
      }
      if (lfsz != 0) {
        fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i)
          next_frontier[fstart+i] = lf[i];
      }
    }
    else{
      BottomUpStep( curr_front_bm, nxt_front_bm, distances)
    }
    #pragma omp barrier
    
    #pragma omp single
    { 
      is_top_down = (curr_frontier_size > 0.05 * N)? true : false ;
      swap(curr_frontier, next_frontier);
      swap(curr_front_bm, nxt_front_bm);
      fsz = nxt_fsz;
      nxt_fsz = 0;
      depth++;
    }
    #pragma omp barrier
    if(is_TD_2_BU){
      //convert local frontiers to bitmap(curr_front_bm)
    }
    else if(is_BU_2_TD){
      // convert bitmap to frontier(curr_frontier)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}
\FloatBarrier

==> optimizations_bkp1.tex <==
\section{Optimization Strategies}
\label{sec:optimizations}

In this section, we describe several optimizations to improve the performance of parallel BFS on multicore processors. We present these optimizations in the context of the parallel BFS kernel shown in Listing~\ref{lst:bfs_v1} (excluding the highlighted code block in blue). We refer to this kernel as the \texttt{BFS-Conventional} kernel, which uses atomic operations to ensure single-threaded updates to vertex distances.

Throughout our discussion of optimizations, the term 'local frontier' refers to the vertices collected by each individual thread during an iteration, before they are merged into the global frontier. While we experimented with various parallel scheduling approaches, including dynamic scheduling with different chunk sizes, static scheduling consistently showed the best average performance on the Speedcode platform~\cite{speedcode} in our experiments.

~\\
\noindent \textbf{\texttt{BFS-NonAtomic:}} In the \texttt{BFS-Conventional} kernel, we use atomic operations to update vertex distances. These atomic operations are expensive and can lead to contention. In our bulk-synchronous BFS implementation, since threads update vertex distances synchronously level by level, a vertex's distance is updated with the same value even when multiple threads attempt to update it. Removing atomic updates introduces two issues: (1) Duplicate work: The same vertex can be added to the frontier multiple times by different threads, leading to redundant processing in the next iteration, (2) Data races: Since multiple threads update the same memory location without synchronization, this creates a data race according to the C++11 standard, which defines it as concurrent conflicting actions where at least one is non-atomic. (Section 1.10.21 in~\cite{cpp:standard}). While multiple threads updating the same memory location without synchronization is technically undefined behavior according to the C++ standard, our implementation exploits the fact that all concurrent updates write the same distance value due to the level-synchronized nature of BFS. In Section~\ref{sec:evaluation}, we quantify the performance impact of this optimization and caution that its usage should be limited to architectures that provide the necessary hardware guarantees and contexts where compiler optimizations won't affect the intended behavior. Also note that this optimization is specific to BFS's distance updates and cannot be employed if a node's data must be strictly updated only once.

In Figure~\ref{fig:avg_duplicates} (left), we show the average percentage of duplicates in the frontier across iterations without atomic updates. We observe that the percentage of duplicates is less than $1\%$ of the total frontier size across several datasets. The dataset \texttt{kNN\_graph} has the highest average duplicates at $31.6\%$. Figures~\ref{fig:avg_duplicates} (middle and right) show the percentage of duplicates and frontier sizes across iterations for the \texttt{kNN\_graph}, respectively. We observe that the percentage of duplicates increases in later iterations when the frontier size becomes small (less than $1\%$ of total vertices). Therefore, although the percentage of duplicates appears high, the actual number of duplicate vertices is small. Since many threads would be idle during these small-frontier iterations anyway, having them process duplicate vertices does not negatively impact performance.

\begin{figure*}
    \centering
    \includegraphics[scale=0.41]{figures/duplicates.pdf}
    \vspace{-2mm}
    %\hrule
    \caption{Analysis of duplicates and frontier size across iterations.}
    \label{fig:avg_duplicates}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 1 //Pure Top-Down with Locks, thread launched only once
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v1,caption=Parallel BFS kernel showing both atomic and non-atomic distance updates.]
#pragma omp parallel
{
  while (cfsz != 0) {
    // Traverse all vertices in current frontier
    #pragma omp for nowait
    for (uint32_t i = 0; i < cfsz; ++i) {
      vidType src = curr_frontier[i];
      // Traverse all neighbors of frontier vertex
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
        vidType dst = col[j];
        // if neighbor is not visited
        if (dist[src] + 1 < dist[dst]) {
          // |\color{darkred}{BFS-Conventional: atomically update the neighbor's distance}|
          |\vspace{-0.8em}|
          |\vspace{0.8em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=2.45]{codebox}
          if (\_\_sync\_bool\_compare\_and\_swap(\&dist[dst], MAX\_DISTANCE, dist[src] + 1)) \{
          \tikzmarkend{codebox} |

          // |\color{darkred}{BFS-NonAtomic: Update the distance directly. See issue 2 as detailed in \texttt{BFS-NonAtomic}}|
          |\vspace{-0.8em}|
          |\vspace{0.3em} \tikzmarkin[set fill color=lightblue, set border color=white, above offset=0.22, below offset=-0.1, right offset=3.62]{codebox3}
          dist[dst] = dist[src] + 1;
          \tikzmarkend{codebox3} |

            // Add to local frontier
            lf[lfsz++] = dst;
          |\vspace{0.6em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=6.6]{codebox2}
          \}
          \tikzmarkend{codebox2} |
        }
      }
    }
    if (lfsz != 0) {
      // collect local frontiers
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        next_frontier[fstart+i] = lf[i];
    }
    #pragma omp barrier
    
    #pragma omp single
    {
      swap(curr_frontier, next_frontier);
      cfsz = nxt_fsz; nxt_fsz = 0;
    }
    lfsz = 0;
  }
}
\end{lstlisting}
\vspace{-0.09in}
\noindent \textbf{\texttt{BFS-Hybrid:}} In~\cite{beamer:direction-optimizing}, the authors propose a hybrid BFS algorithm that dynamically switches between top-down and bottom-up phases based on frontier size. The top-down phase is used when the frontier is small, while the bottom-up phase is employed when it's large. In the bottom-up phase, for each unvisited vertex, the algorithm checks if any of its neighbors are in the current frontier. If so, the unvisited vertex's distance is updated and it's added to the next frontier. This optimization reduces the number of edges traversed. The switching criteria in~\cite{beamer:direction-optimizing} is based on the next frontier edges to be visited ($m_f$), total unvisited edges ($m_u$), and next frontier size ($f_{i+1}$). The algorithm switches from top-down to bottom-up when $m_f > m_u / \alpha$, and switches back when $f_{i+1} < N / \beta$ and $f_{i+1} < f_i$. $\alpha$ and $\beta$ are tuning parameters.
We refer to this as $\texttt{BFS-Hybrid}^{\dagger}$. We simplify these criteria to use only the next frontier size, eliminating the need to compute and synchronize $m_f$ and $m_u$ across threads. Our version, which we call $\texttt{BFS-Hybrid}$, switches phases when the frontier size crosses $5\%$ of the total vertices and is detailed in Listing~\ref{lst:bfs_v3}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 3 //Hybrid(Top-Down + Bottom-Up)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v3,caption=Hybrid parallel BFS kernel with dynamic switching between top-down and bottom-up phases]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down) {
      // Same as |Listing: \ref{lst:bfs_v1}|
    }
    else{
      // Frontiers are collected in a bitmap
      // Reset nxt_front_bm
      #pragma omp for nowait reduction(+: nxt_fsz)
      for (vidType v = 0; v < N; v++) { 
        if (dist[v] == MAX_DISTANCE) { 
          // Check if its neighbors are in the current frontier
          for (uint32_t j = rptr[v]; j < rptr[v+1]; ++j) {
            vidType neighbor = col[j];
            if (curr_front_bm[neighbor]) {
              dist[v] = depth + 1;
              nxt_fsz++;
              nxt_front_bm[v] = true;
              break;
            }
          }
        }
      }
    }
    #pragma omp barrier
    #pragma omp single
    { 
      // update curr_frontier, curr_front_bm, cfsz and nxt_fsz
      is_top_down = (cfsz < 0.05 * N)? true : false;
      depth++;
    }
    #pragma omp barrier
    if(move_from_TD_to_BU) {
      // convert  frontier array to curr_front_bm (bitmap)
    }
    else if(move_from_BU_to_TD) {
      // convert curr_front_bm (bitmap) to curr_frontier (array)
    }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}
\vspace{-0.09in}

\noindent \textbf{\texttt{BFS-VisitedBitmap:}} The \texttt{BFS-Hybrid} relies on the distance array to check visited vertices in both phases. These random accesses to the distance array can lead to cache misses. Moreover, loading a 4- or 8-byte integer from memory just to check if a vertex is visited is inefficient. We propose using a bitmap to track visited vertices instead, an optimization we call \texttt{BFS-VisitedBitmap}. Listing~\ref{lst:bfs_v5} shows how this bitmap tracks visited vertices, where the distance array is accessed and updated only when a vertex is found to be unvisited.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v5,caption=Hybrid parallel BFS kernel using bitmap for visited vertex tracking]
// Use a bitmap to check if a vertex is visited
// In top-down
for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
  vidType dst = col[j];
  if (!visited_bm[dst]) {
    dist[dst] = dist[src] + 1;
    lf[lfsz++] = dst;
    visited_bm[dst] = true;
  }
}
// In bottom-up
#pragma omp for nowait reduction(+: nxt_fsz)
for (vidType v = 0; v < N; v++) { 
  if (!visited_bm[v]) { 
    for (uint32_t j = rptr[v]; j < rptr[v+1]; ++j) {
      vidType neighbor = col[j];
      if (curr_front_bm[neighbor]) {
        dist[v] = depth + 1;
        nxt_fsz++;
        nxt_front_bm[v] = true;
        visited_bm[v] = true;
        break;
      }
    }
  }
}
// Optimize further to avoid random accesses. For example, in the top-down phase
for (uint32_t i = 0; i < cfsz; ++i) {
  vidType src = curr_frontier[i];
  for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
    vidType dst = col[j];
    if (!visited_bm[dst]) {
      lf[lfsz++] = dst;
      visited_bm[dst] = true;
    }
  }
}
sort(lf, lf + lfsz);
for (uint32_t i = 0; i < lfsz; ++i) {
  dist[lf[i]] = depth + 1;
}
\end{lstlisting}
%\vspace{-0.1in}
%\footnote{According to the C++11 standard draft \cite{ISO:2013:N3690}, a data race is defined as "The execution of a program contains a data race if it contains two conflicting actions in different threads, at least one of which is not atomic, and neither happens before the other."}

This optimization can be extended further to eliminate random memory accesses entirely. The code block between lines 27-38 in Listing~\ref{lst:bfs_v5} demonstrates this approach. The loop now only accesses the visited bitmap. After the loop completes, the local frontier is sorted and distances are updated in order. When the visited bitmap fits in cache, and the size of the local frontier is small, this optimization leads to better cache utilization and fewer memory accesses.

~\\
\noindent \textbf{\texttt{Other Optimizations:}} Among various optimizations we explored, we highlight three key approaches, though none yielded performance gains in our experiments. (a) In the top-down phase, we implemented periodic flushing of local frontiers to the global frontier,  
%(Listing~\ref{lst:bfs_v8})
similar to an optimization in~\cite{beamer:direction-optimizing}. This approach limits local frontier sizes thereby reducing the memory overhead, 
(b) For the bottom-up phase, we employed SIMD instructions to vectorize the neighbor-checking loop and introduced prefetch requests for the \texttt{col} and \texttt{curr\_front\_bm} arrays to minimize cache misses, (c) In the top-down phase, when the global frontier reaches a sufficient size, we distribute work among threads and allow them to process independently without merging local frontiers, either for several iterations or until the global frontier size decreases below a threshold. This optimization reduces synchronization overhead and eliminates bulk memory copies from local to global frontiers.

\if 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 8
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v8,caption=Hybrid parallel BFS kernel with periodic frontier flushing in top-down phase]
// in top-down
#pragma omp for nowait
for (uint32_t i = 0; i < cfsz; ++i) {
  vidType src = curr_frontier[i];
  for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
    vidType dst = col[j];
    if (dist[src] + 1 < dist[dst]) {
      dist[dst] = dist[src] + 1;
      lf[lfsz++] = dst;
      // periodically flush local frontier
      if(lfsz == max_lfsz){
        f_start = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i) {
          next_frontier[f_start + i] = lf[i];
        }
        lfsz = 0;
      }
    }
  }
}
// flush remaining local frontier if lfsz is not zero
\end{lstlisting}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 7
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v7,caption=Hybrid parallel BFS kernel with SIMD-vectorized bottom-up phase]
// in bottom-up
__m256i depth_vec = _mm256_set1_epi32(depth);
if(dist[v] == MAX_DISTANCE) {
  bool is_parent = false;
  uint32_t i_end = rptr[v] + ((rptr[v+1] - rptr[v]) / chunksize) * chunksize;
  for (uint32_t i = rptr[v]; i < i_end; i += chunksize) {
    _mm_prefetch((const char*)&col[i+chunksize], _MM_HINT_T0);
    _mm_prefetch((const char*)&curr_front_bm[col[i + chunksize]], _MM_HINT_T0);
    for (uint32_t j = i; j < i + chunksize; j += 8) {
      __m256i parent_vec = _mm256_loadu_si256((__m256i*)&col[j]);
      __m256i distances_vec = _mm256_i32gather_epi32((int const*)dist, parent_vec, 4);                          
      __m256i cmp_result = _mm256_cmpeq_epi32(distances_vec, depth_vec);
      if (_mm256_movemask_epi8(cmp_result)) {
        is_parent = true;
      }
    }
    if(is_parent) {
      dist[v] = depth + 1;
      nxt_fsz++;
      nxt_front_bm[v] = true;
      break;
    }
  }
  // Handle the remainder of the loop
}
\end{lstlisting}
\vspace{-0.1in}
\fi



==> optimizations_bkp2.tex <==
\section{Optimization Strategies}
\label{sec:optimizations}

In this section, we describe several optimizations to improve the performance of parallel BFS on multicore processors. We present these optimizations in the context of the parallel BFS kernel shown in Listing~\ref{lst:bfs_v1} (excluding the highlighted code block in blue). We refer to this kernel as the \texttt{BFS-Conventional} kernel, which uses atomic operations to ensure single-threaded updates to vertex distances.

Throughout our discussion of optimizations, the term 'local frontier' refers to the vertices collected by each individual thread during an iteration, before they are merged into the global frontier. While we experimented with various parallel scheduling approaches, including dynamic scheduling with different chunk sizes, static scheduling consistently showed the best average performance on the Speedcode platform~\cite{speedcode} in our experiments.

~\\
\noindent \textbf{\texttt{BFS-NonAtomic:}} In the \texttt{BFS-Conventional} kernel, we use atomic operations to update vertex distances. These atomic operations are expensive and can lead to contention. In our bulk-synchronous BFS implementation, since threads update vertex distances synchronously level by level, a vertex's distance is updated with the same value even when multiple threads attempt to update it. Removing atomic updates introduces two issues: (1) Duplicate work: The same vertex can be added to the frontier multiple times by different threads, leading to redundant processing in the next iteration, (2) Data races: Since multiple threads update the same memory location without synchronization, this creates a data race according to the C++11 standard, which defines it as concurrent conflicting actions where at least one is non-atomic. (Section 1.10.21 in~\cite{cpp:standard}). While multiple threads updating the same memory location without synchronization is technically undefined behavior according to the C++ standard, our implementation exploits the fact that all concurrent updates write the same distance value due to the level-synchronized nature of BFS. In Section~\ref{sec:evaluation}, we quantify the performance impact of this optimization and caution that its usage should be limited to architectures that provide the necessary hardware guarantees and contexts where compiler optimizations won't affect the intended behavior. Also note that this optimization is specific to BFS's distance updates and cannot be employed if a node's data must be strictly updated only once.

In Figure~\ref{fig:avg_duplicates} (left), we show the average percentage of duplicates in the frontier across iterations without atomic updates. We observe that the percentage of duplicates is less than $1\%$ of the total frontier size across several datasets. The dataset \texttt{kNN\_graph} has the highest average duplicates at $31.6\%$. Figures~\ref{fig:avg_duplicates} (middle and right) show the percentage of duplicates and frontier sizes across iterations for the \texttt{kNN\_graph}, respectively. We observe that the percentage of duplicates increases in later iterations when the frontier size becomes small (less than $1\%$ of total vertices). Therefore, although the percentage of duplicates appears high, the actual number of duplicate vertices is small. Since many threads would be idle during these small-frontier iterations anyway, having them process duplicate vertices does not negatively impact performance.

\begin{figure*}
    \centering
    \includegraphics[scale=0.41]{figures/duplicates.pdf}
    \vspace{-2mm}
    %\hrule
    \caption{Analysis of duplicates and frontier size across iterations.}
    \label{fig:avg_duplicates}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 1 //Pure Top-Down with Locks, thread launched only once
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v1,caption=Parallel BFS kernel showing both atomic and non-atomic distance updates.]
#pragma omp parallel
{
  while (cfsz != 0) {
    // Traverse all vertices in current frontier
    #pragma omp for nowait
    for (uint32_t i = 0; i < cfsz; ++i) {
      vidType src = curr_frontier[i];
      // Traverse all neighbors of frontier vertex
      for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
        vidType dst = col[j];
        // if neighbor is not visited
        if (dist[src] + 1 < dist[dst]) {
          // |\color{darkred}{BFS-Conventional: atomically update the neighbor's distance}|
          |\vspace{-0.8em}|
          |\vspace{0.8em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=2.45]{codebox}
          if (\_\_sync\_bool\_compare\_and\_swap(\&dist[dst], MAX\_DISTANCE, dist[src] + 1)) \{
          \tikzmarkend{codebox} |

          // |\color{darkred}{BFS-NonAtomic: Update the distance directly. See issue 2 as detailed in \texttt{BFS-NonAtomic}}|
          |\vspace{-0.8em}|
          |\vspace{0.3em} \tikzmarkin[set fill color=lightblue, set border color=white, above offset=0.22, below offset=-0.1, right offset=3.62]{codebox3}
          dist[dst] = dist[src] + 1;
          \tikzmarkend{codebox3} |

            // Add to local frontier
            lf[lfsz++] = dst;
          |\vspace{0.6em} \tikzmarkin[set fill color=lightgrey, set border color=white, above offset=0.22, below offset=-0.1, right offset=6.6]{codebox2}
          \}
          \tikzmarkend{codebox2} |
        }
      }
    }
    if (lfsz != 0) {
      // collect local frontiers
      fstart = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
      for (uint32_t i = 0; i < lfsz; ++i)
        next_frontier[fstart+i] = lf[i];
    }
    #pragma omp barrier
    
    #pragma omp single
    {
      swap(curr_frontier, next_frontier);
      cfsz = nxt_fsz; nxt_fsz = 0;
    }
    lfsz = 0;
  }
}
\end{lstlisting}
\vspace{-0.09in}
\noindent \textbf{\texttt{BFS-Hybrid:}} In~\cite{beamer:direction-optimizing}, the authors propose a hybrid BFS algorithm that dynamically switches between top-down and bottom-up phases based on frontier size. The top-down phase is used when the frontier is small, while the bottom-up phase is employed when it's large. In the bottom-up phase, for each unvisited vertex, the algorithm checks if any of its neighbors are in the current frontier. If so, the unvisited vertex's distance is updated and it's added to the next frontier. This optimization reduces the number of edges traversed. The switching criteria in~\cite{beamer:direction-optimizing} is based on the next frontier edges to be visited ($m_f$), total unvisited edges ($m_u$), and next frontier size ($f_{i+1}$). The algorithm switches from top-down to bottom-up when $m_f > m_u / \alpha$, and switches back when $f_{i+1} < N / \beta$ and $f_{i+1} < f_i$. $\alpha$ and $\beta$ are tuning parameters.
We refer to this as $\texttt{BFS-Hybrid}^{\dagger}$. We simplify these criteria to use only the next frontier size, eliminating the need to compute and synchronize $m_f$ and $m_u$ across threads. Our version, which we call $\texttt{BFS-Hybrid}$, switches phases when the frontier size crosses $5\%$ of the total vertices and is detailed in Listing~\ref{lst:bfs_v3}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 3 //Hybrid(Top-Down + Bottom-Up)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v3,caption=Hybrid parallel BFS kernel with dynamic switching between top-down and bottom-up phases]
is_top_down = true;
#pragma omp parallel
{
  while (cfsz != 0) {
    if(is_top_down) {
      // Same as |Listing: \ref{lst:bfs_v1}| }
    else{
      // Frontiers are collected in a bitmap
      // Reset nxt_front_bm
      #pragma omp for nowait reduction(+: nxt_fsz)
      for (vidType v = 0; v < N; v++) { 
        if (dist[v] == MAX_DISTANCE) { 
          // Check if its neighbors are in the current frontier
          for (uint32_t j = rptr[v]; j < rptr[v+1]; ++j) {
            vidType neighbor = col[j];
            if (curr_front_bm[neighbor]) {
              dist[v] = depth + 1;
              nxt_fsz++;
              nxt_front_bm[v] = true;
              break; } } } } }
    #pragma omp barrier
    #pragma omp single
    { 
      // update curr_frontier, curr_front_bm, cfsz and nxt_fsz
      is_top_down = (cfsz < 0.05 * N)? true : false;
      depth++;
    }
    #pragma omp barrier
    if(move_from_TD_to_BU) {
      // convert  frontier array to curr_front_bm (bitmap) }
    else if(move_from_BU_to_TD) {
      // convert curr_front_bm (bitmap) to curr_frontier (array) }
    lfsz = 0;
    #pragma omp barrier
  }
}
\end{lstlisting}
\vspace{-0.09in}

\noindent \textbf{\texttt{BFS-VisitedBitmap:}} The \texttt{BFS-Hybrid} relies on the distance array to check visited vertices in both phases. These random accesses to the distance array can lead to cache misses. Moreover, loading a 4- or 8-byte integer from memory just to check if a vertex is visited is inefficient. We propose using a bitmap to track visited vertices instead, an optimization we call \texttt{BFS-VisitedBitmap}. Listing~\ref{lst:bfs_v5} shows how this bitmap tracks visited vertices, where the distance array is accessed and updated only when a vertex is found to be unvisited.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v5,caption=Hybrid parallel BFS kernel using bitmap for visited vertex tracking]
// Use a bitmap to check if a vertex is visited
// In top-down
for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
  vidType dst = col[j];
  if (!visited_bm[dst]) {
    dist[dst] = dist[src] + 1;
    lf[lfsz++] = dst;
    visited_bm[dst] = true; } }
// In bottom-up
#pragma omp for nowait reduction(+: nxt_fsz)
for (vidType v = 0; v < N; v++) { 
  if (!visited_bm[v]) { 
    for (uint32_t j = rptr[v]; j < rptr[v+1]; ++j) {
      vidType neighbor = col[j];
      if (curr_front_bm[neighbor]) {
        dist[v] = depth + 1;
        nxt_fsz++;
        nxt_front_bm[v] = visited_bm[v] = true;
        break; } } }
// Optimize further to avoid random accesses. For example, in the top-down phase
for (uint32_t i = 0; i < cfsz; ++i) {
  vidType src = curr_frontier[i];
  for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
    vidType dst = col[j];
    if (!visited_bm[dst]) {
      lf[lfsz++] = dst;
      visited_bm[dst] = true;
    }
  }
}
sort(lf, lf + lfsz);
for (uint32_t i = 0; i < lfsz; ++i) {
  dist[lf[i]] = depth + 1;
}
\end{lstlisting}
%\vspace{-0.1in}
%\footnote{According to the C++11 standard draft \cite{ISO:2013:N3690}, a data race is defined as "The execution of a program contains a data race if it contains two conflicting actions in different threads, at least one of which is not atomic, and neither happens before the other."}

This optimization can be extended further to eliminate random memory accesses entirely. The code block between lines 27-38 in Listing~\ref{lst:bfs_v5} demonstrates this approach. The loop now only accesses the visited bitmap. After the loop completes, the local frontier is sorted and distances are updated in order. When the visited bitmap fits in cache, and the size of the local frontier is small, this optimization leads to better cache utilization and fewer memory accesses.

~\\
\noindent \textbf{\texttt{Other Optimizations:}} Among various optimizations we explored, we highlight three key approaches, though none yielded performance gains in our experiments. (a) In the top-down phase, we implemented periodic flushing of local frontiers to the global frontier,  
%(Listing~\ref{lst:bfs_v8})
similar to an optimization in~\cite{beamer:direction-optimizing}. This approach limits local frontier sizes thereby reducing the memory overhead, 
(b) For the bottom-up phase, we employed SIMD instructions to vectorize the neighbor-checking loop and introduced prefetch requests for the \texttt{col} and \texttt{curr\_front\_bm} arrays to minimize cache misses, (c) In the top-down phase, when the global frontier reaches a sufficient size, we distribute work among threads and allow them to process independently without merging local frontiers, either for several iterations or until the global frontier size decreases below a threshold. This optimization reduces synchronization overhead and eliminates bulk memory copies from local to global frontiers.

\if 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 8
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v8,caption=Hybrid parallel BFS kernel with periodic frontier flushing in top-down phase]
// in top-down
#pragma omp for nowait
for (uint32_t i = 0; i < cfsz; ++i) {
  vidType src = curr_frontier[i];
  for (uint32_t j = rptr[src]; j < rptr[src+1]; ++j) {
    vidType dst = col[j];
    if (dist[src] + 1 < dist[dst]) {
      dist[dst] = dist[src] + 1;
      lf[lfsz++] = dst;
      // periodically flush local frontier
      if(lfsz == max_lfsz){
        f_start = __atomic_fetch_add(&nxt_fsz, lfsz, __ATOMIC_SEQ_CST);
        for (uint32_t i = 0; i < lfsz; ++i) {
          next_frontier[f_start + i] = lf[i];
        }
        lfsz = 0;
      }
    }
  }
}
// flush remaining local frontier if lfsz is not zero
\end{lstlisting}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%version 7
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lstlisting}[aboveskip=0em, belowskip=0em, float=!h,label=lst:bfs_v7,caption=Hybrid parallel BFS kernel with SIMD-vectorized bottom-up phase]
// in bottom-up
__m256i depth_vec = _mm256_set1_epi32(depth);
if(dist[v] == MAX_DISTANCE) {
  bool is_parent = false;
  uint32_t i_end = rptr[v] + ((rptr[v+1] - rptr[v]) / chunksize) * chunksize;
  for (uint32_t i = rptr[v]; i < i_end; i += chunksize) {
    _mm_prefetch((const char*)&col[i+chunksize], _MM_HINT_T0);
    _mm_prefetch((const char*)&curr_front_bm[col[i + chunksize]], _MM_HINT_T0);
    for (uint32_t j = i; j < i + chunksize; j += 8) {
      __m256i parent_vec = _mm256_loadu_si256((__m256i*)&col[j]);
      __m256i distances_vec = _mm256_i32gather_epi32((int const*)dist, parent_vec, 4);                          
      __m256i cmp_result = _mm256_cmpeq_epi32(distances_vec, depth_vec);
      if (_mm256_movemask_epi8(cmp_result)) {
        is_parent = true;
      }
    }
    if(is_parent) {
      dist[v] = depth + 1;
      nxt_fsz++;
      nxt_front_bm[v] = true;
      break;
    }
  }
  // Handle the remainder of the loop
}
\end{lstlisting}
\vspace{-0.1in}


